Scalable Online Exploration via Coverability

Exploration is a major challenge in reinforcement learning, especially for high-dimensional domains that require function approximation. We propose exploration objectives -- policy optimization objectives that enable downstream maximization of any reward function -- as a conceptual framework to systematize the study of exploration. Within this framework, we introduce a new objective, $L_1$-Coverage, which generalizes previous exploration schemes and supports three fundamental desiderata: 1. Intrinsic complexity control. $L_1$-Coverage is associated with a structural parameter, $L_1$-Coverability, which reflects the intrinsic statistical difficulty of the underlying MDP, subsuming Block and Low-Rank MDPs. 2. Efficient planning. For a known MDP, optimizing $L_1$-Coverage efficiently reduces to standard policy optimization, allowing flexible integration with off-the-shelf methods such as policy gradient and Q-learning approaches. 3. Efficient exploration. $L_1$-Coverage enables the first computationally efficient model-based and model-free algorithms for online (reward-free or reward-driven) reinforcement learning in MDPs with low coverability. Empirically, we find that $L_1$-Coverage effectively drives off-the-shelf policy optimization algorithms to explore the state space.

==> scratch.tex <==
\section*{Scratch}

\paragraph{Notation}
\begin{itemize}
\item MDPs:
  \begin{itemize}
  \item Not layered is the current plan.
  \item \dfcomment{Suppress dependence on $\Mstar$ when the model is fixed.}
  \end{itemize}
\item Coverability:
  \begin{itemize}
  \item 
  \end{itemize}
\item Occupancies:
  \begin{itemize}
  \item Definitely want to use $d^{p}$ abbreviation
  \end{itemize}
\item Follow constrained DEC notation: For reward-free, we gather data
  with $q$ and output $p$. For reward-based/regret, we gather data and
  output $p$.
\end{itemize}

\subsection*{Organization}

  \dfcomment{New plan for section:
    \begin{enumerate}
    \item Begin by introducing our main objective: $L_2$ coverability.
      \begin{itemize}
      \item Writing questions:
        \begin{itemize}
        \item What to name this notion of coverability?
        \item What do name what it is ``exploration objective'',
          ``notion of coverage?''?
          \begin{itemize}
          \item Intuitively, a policy cover should have good
            coverage. We define an exploration objective as something
            you optimize in order to learn a policy with good
            coverage. (What does the PC-PG paper say here?)
          \end{itemize}
        \end{itemize}
      \end{itemize}
    \item Explain that several existing notions of coverage are
      subsumed by it:
      \begin{itemize}
      \item $L_{\infty}$ coverability (non-realizable)
      \item Feature coverage (non-realizable)
      \item Non-realizable $L_2$? Need to check.
      \end{itemize}
    \item Show that it's sufficient for downstream offline RL.
    \item Mention that other notions (realizable $L_{\infty}$) are insufficient 
    \end{enumerate}
    }


  \begin{align}
    \CovM(p) =
    \sup_{\pi\in\Pi}\En^{\sM,\pi}\brk*{\frac{d^{\sM,\pi}_h(x_h,a_h)}{d_h^{\sM,p}(x_h,a_h)+\veps\cdot{}d_h^{\sM,\pi}(x_h,a_h)}},
    \mathand \CovOptM = \inf_{p\in\Delta(\Pi)}\CovM(p).
  \end{align}
  When the MDP $M$ is clear from context, we drop the dependence on $M$
  and write $\Cov(p)\equiv\CovM(p)$, $\CovOpt\equiv\CovOptM$, and so
  forth.

  For distributions $\mu\in\Delta(\cX\times\cA)$, we write
  \begin{align}
    \CovNRM(\mu) =
    \sup_{\pi\in\Pi}\En^{\sM,\pi}\brk*{\frac{d_h^{\sM,\pi}(x_h,a_h)}{\mu(x_h,a_h)+\veps\cdot{}d_h^{\sM,\pi}(x_h,a_h)}},
    \mathand \CovNROptM = \inf_{\mu\in\Delta(\cX\times\cA)}\CovNRM(\mu).
  \end{align}


\paragraph{$L_\infty$ coverability}  
    \begin{align}
    \ICovM(p) =
    \sup_{\pi\in\Pi}\sup_{(x,a)\in\cX\times\cA}\crl*{\frac{d^{\sM,\pi}_h(x,a)}{d_h^{\sM,p}(x,a)+\veps\cdot{}d_h^{\sM,\pi}(x,a)}},
    \mathand \ICovOptM = \inf_{p\in\Delta(\Pi)}\ICovM(p).
    \end{align}

    For distributions $\mu\in\Delta(\cX\times\cA)$, we write
  \begin{align}
    \ICovNRM(\mu) =
    \sup_{\pi\in\Pi}\sup_{(x,a)\in\cX\times\cA}\crl*{\frac{d_h^{\sM,\pi}(x_h,a_h)}{\mu(x_h,a_h)+\veps\cdot{}d_h^{\sM,\pi}(x_h,a_h)}},
    \mathand \ICovNROptM = \inf_{\mu\in\Delta(\cX\times\cA)}\ICovNRM(\mu).
  \end{align}

  \paragraph{Pushforward coverability}  
    \begin{align}
    \PCovM(p) =
    \sup_{\pi\in\Pi}\sup_{(x,a)\in\cX\times\cA}\crl*{\frac{d^{\sM,\pi}_h(x,a)}{d_h^{\sM,p}(x,a)+\veps\cdot{}d_h^{\sM,\pi}(x,a)}},
    \mathand \PCovOptM = \inf_{p\in\Delta(\Pi)}\PCovM(p).
    \end{align}

    For distributions $\mu\in\Delta(\cX)$, we write
  \begin{align}
    \PCovNRM(\mu) =
\sup_{\pi\in\Pi}\sup_{(x,a,x')\in\cX\times\cA\times\cX}\crl*{\frac{P^{\sM}_h(x'\mid{}x,a)}{\mu(x')+\veps\cdot{}P_h^{\sM}(x'\mid{}x,a)}},
    \mathand \PCovNROptM = \inf_{\mu\in\Delta(\cX\times\cA)}\PCovNRM(\mu).
  \end{align}

\paragraph{Relaxations}
    
    \begin{align}
    \CovM(p) =
    \sup_{\pi\in\Pi}\En^{\sM,\pi}\brk*{\frac{d^{\sM,\pi}_h(x_h,a_h)}{d_h^{\sM,p}(x_h,a_h)+\veps\cdot{}d_h^{\sM,\pi}(x_h,a_h)}},
    \mathand \CovOptM = \inf_{p\in\Delta(\Pi)}\CovM(p).
  \end{align}

~\\~\\~\\  
  \begin{itemize}
  \item $L_2$-Coverability, realizable. 
    \begin{itemize}
    \item $\cov_{2,\veps}(p)$, $\cov^{\sM}_{2,\veps}(p)$
    \item  Or, $\cov_\veps(p)$, $\cov^{\sM}_\veps(p)$
      (drop the $2$ since this is our main quantity).
    \item Could make the first displayed eq just $\cov(p)$
      ($\veps=0$), then define $\veps$ version after.
      \item Optimal value: $\cov_{\veps}^{\star}$ or
        $\cov_{\veps}^{\sM,\star}$ or $\cov^{\star}_\veps(M)$? Not a big fan of how this
        looks with $M$.
        \begin{itemize}
        \item Potentially a non-issue if we suppress dependence on
          $\Mstar$, except when we need to write this for
          $\Mhat\ind{t}$ etc explicitly. Otoh, i kinda of like the
          idea of doing this whole section with a fixed $M$ and making 
          dependence explicit.
        \item Another idea:  Optimal value is just
          $C=\inf_p\cov(p)$ or similar, can write
          $C(M)=\inf_p\cov^{\sM}(p)$ or similar.
        \end{itemize}
      \item $L_{\infty}$ version: $\cov_\infty(p)$,
        $\cov^{\sM}_\infty(p)$ (overloads w/ $\veps$ above)
      \item Other ideas:
        \begin{itemize}
        \item $\cov(p; \veps)$, $\cov_\infty(p; \veps)$,
          $\cov(p; \veps, M)$, $\cov_\infty(p; \veps, Me)$
        \item Opt becomes $\cov^{\star}(\veps)$ which is kinda weird.
         \item  Or, $\textsf{cov}_\veps(p)$,
          $\textsf{cov}^{\sM}_\veps(p)$ etc \dfcomment{idea: lowercase
            for realizable, uppercase for non-realizable}
        \end{itemize}
      \end{itemize}
    \item We say that $p$ is a $(C,\veps)$-cover if $\cov_{2,\veps}(p)\leq{}C$.
    \item Non-realizable coverability: Just underline.
      \begin{itemize}
      \item $L_2$: $\covu_\veps(\mu)$ etc. \dfcomment{used almost
          nowhere so not a big deal}
      \item $L_{\infty}$: $\covu_\infty(\mu)$,
        $\covu_\infty^{\star}$. \dfcomment{this one is
          important/fundamental so it should be short ideally.}
      \end{itemize}
    \item $\mu$-based relaxation:
      \begin{itemize}
      \item $\textsf{$\mu$-cov}$
        \item $\wb{\cov}_{\veps}(p;\mu)$ or $\wb{\cov}_{\veps;\mu}(p)$.
      \end{itemize}
    \item Pushforward relaxation
      \begin{itemize}
      \item $\wt{\cov}_{\veps}(p)$, but otherwise keep all the
        notation the same?
      \item Pushforward coverability $\textsf{PCov}$ or $\textsf{pcov}$?
      \end{itemize}
    \item Note: For both relaxations, need succinct definition for 1)
      optimal non-realizable $L_{\infty}$ conc ($\textsf{Cov}_{\infty}^{\star}$?) 2) optimal
      non-realizable pushforward conc
      ($\textsf{PCov}_{\infty}^{\star}$?)
      \begin{itemize}
      \item We could also go back to defining $C_{\textsf{cov}}$,
        $C_{\textsf{push}}$, etc as the optimal value for these things.
      \end{itemize}
    \item Quantities that actually matter
      \begin{itemize}
      \item Realizable $L_2$ (value and opt)
      \item Non-realizable $L_\infty$ opt.
      \item Non-realizable pushforward opt.
      \item $\mu$-based relaxation and pushforward relaxation (value
        and opt)
      \end{itemize}
  \end{itemize}

  


==> section_model_free-arxiv.tex <==
\pacomment{copied the model-free section from the appendix. should we trim this down a bit?}

\pacomment{ideas for this section:
\begin{itemize}
	\item weight function assumption: only give strong version of assumptions (tease weak version?)
	\item shorten weight function estimation: pseudocode in the appendix, less motivation.
	\item policy optimization section: psdp only?
	\item main guarantee: psdp only?
\end{itemize}
}

Our algorithms in the previous section show that the \mainobj
objective and \mainopt parameter enable sample-efficient online
reinforcement learning, but one potential drawback is that they
require model-based realizability, a strong form of function
approximation that may not always be realistic. In this section, we
give \emph{model-free} algorithms to perform reward-free exploration
and optimize the \mainobj objective that do not require model
realizability, and instead require a weaker form of \emph{density
  ratio} or \emph{weight
  function} realizability, a modeling
approach that has been widely used in offline reinforcement learning \citep{liu2018breaking,uehara2020minimax,yang2020off,uehara2021finite,jiang2020minimax,xie2020q,zhan2022offline,chen2022offline,rashidinejad2022optimal,ozdaglar2023revisiting}
and recently adapted to the online setting
\citep{amortila2023harnessing}. The main algorithm we present achieves
\paedit{a bound we give on the \mainobj
value scales with the pushforward coverability parameter
$\CpushM[\Mstar]$} \pacomment{what?}, which is weaker than the guarantee achieved by our
model-based algorithms, but the weaker modeling assumptions make it
applicable in a broader range of settings. Computationally, the
algorithm reduces to reward-driven policy optimization and a standard supervised
weight function estimation objective.


Throughout this section, we take $\Pi=\PiNS$ as the set of all
non-stationary policies.




\subsection{Algorithm}

\paedit{Our model-free algorithm}, \mfalg, is presented in \cref{alg:model_free}. The
algorithm builds a collection of policy covers
$p_1,\ldots,p_H\in\Delta(\PiRNS)$ layer-by-layer in an inductive
fashion. For each layer $h\in\brk{H}$, given policy
covers $p_1,\ldots,p_{h-1}$ for the preceding layers, the algorithm
computes $p_h$ by (approximately) implementing the iterative algorithm
for policy cover construction given in
\cref{alg:pushforward_relaxation} (\cref{sec:pushforward_relaxation}),
in a data-driven fashion.\icml{\footnote{Note that while the results in
  \cref{sec:planning} are presented
    for the setting in which the underlying MDP $M$ is ``known'' to
    the learner (planning), the algorithmic template in
    \cref{alg:linf_relaxation} can be applied even when $M$ is
    unknown, as long as the policy optimization step in
    \cref{line:linf_opt} can be implemented in a sample-efficient
    fashion. This observation is the basis for the algorithms we
    present in this section.
    }}

In more detail, recall the \emph{pushforward coverability} relaxation
\begin{align*}
    \pCovM[\Mstar](p) =
\sup_{\pi\in\Pi}\En^{\sMstar,\pi}\brk*{\frac{P_{h-1}^{\sMstar}(x_h\mid{}x_{h-1},a_{h-1})}{d_h^{\sMstar,p}(x_h)+\veps\cdot{}P^{\sMstar}_{h-1}(x_h\mid{}x_{h-1}a_{h-1})}}
\end{align*}
for the \mainobj objective given in \cref{sec:pushforward_relaxation}. For layer $h$, \cref{alg:model_free}
approximately minimizes this objective by computing a sequence of policies $\pi\ind{h,1},\ldots,\pi\ind{h,t}$,
where
\begin{align}
\pi\ind{h,t}\approx\argmax_{\pi\in\Pi}\En^{\sMstar,\pi}\brk*{
  \frac{\Pmstar_{h-1}(x_h\mid{}x_{h-1},a_{h-1})}{\sum_{i<t}d_h\ind{\pi\ind{h,i}}(x_h)+\Pmstar_{h-1}(x_h\mid{}x_{h-1},a_{h-1})}}
  \label{eq:mf_argmax}
\end{align}
is computed in fully data-driven/online fashion that makes use of the
preceding policy covers $p_1,\ldots,p_{h-1}$. It then computes the
cover $p_h$ via
$p_h=\unif(\pi\ind{h,1}\circ_h\piunif,\ldots,\pi\ind{h,T}\circ_h\piunif)$.

Our
planning analysis in \cref{sec:pushforward_relaxation} shows that as
long as the approximation error in \cref{eq:mf_argmax} is small, $p_h$
will indeed be an approximate policy cover that minimizes
$\pCovM[\Mstar](p_h)$. To achieve this, \cref{alg:model_free} makes
use of two subroutines. The first subroutine, \estimateweight
(\cref{alg:estimate_weight}), invoked in \cref{line:estimate_weight},
uses function approximation to estimate a weight function
$\what\ind{t}_h$ such that
\begin{align}
  \label{eq:weight_est}
  \what_h\ind{t}(x_h\mid{}x_{h-1},a_{h-1})
  \approx w_h\ind{t}(x_h\mid{}x_{h-1},a_{h-1})
  \ldef{} \frac{\Pmstar_{h-1}(x_h\mid{}x_{h-1},a_{h-1})}{\sum_{i<t}d_h\ind{\pi\ind{h,i}}(x_h)+\Pmstar_{h-1}(x_h\mid{}x_{h-1},a_{h-1})}.
\end{align}
The second subroutine, \policyopt, is a hyperparameter to the algorithm,
and approximately solves the policy optimization problem
\begin{align*}
\pi\ind{h,t}\approx\argmax_{\pi\in\Pi}\En^{\sMstar,\pi}\brk*{
\what_h\ind{t}(x_h\mid{}x_{h-1},a_{h-1})},
\end{align*}
treating the estimated weight function $\what_h\ind{t}$ as a
reward. The \policyopt subroutine can make use of exploratory data
collected using preceding policy
covers $p_1,\ldots,p_{h-1}$, and hence does not have to perform
systematic exploration. Indeed, we show that any hybrid offline/online methods (online methods that require access to
exploratory data) that satisfies a certain ``local'' policy
optimization guarantee is sufficient, with (\psdp{}, \cref{alg:psdp})
\citep{bagnell2003policy} and Natural Policy Gradient
\citep{agarwal2021theory} being natural choices; for our analysis, we make use of \psdp.

\input{algorithm_model_free}


In what follows, we describe the \estimateweight and \policyopt
subroutines and corresponding statistical assumptions in more detail.

\paragraph{Weight function realizability}
To perform weight function estimation, we assume access to a weight function class $\cW=\cW_{1:H}$, with
$\cW_h\subseteq(\cX\times\cA\times\cX\to\bbR_{+})$ that is capable of
representing the weight function $w_h\ind{t}$ in
\cref{eq:weight_est}. In particular, our algorithm is most naturally
stated in terms of the following assumption.
\begin{assumption}[Weight function realizability---strong version]
  \label{ass:weight_realizability_strong}
  For a parameter $T\in\bbN$, we assume that for all $h\geq{}2$, all $t\in\brk{T}$, and all policies
  $\pi\ind{1},\ldots,\pi\ind{t-1}\in\PiNS$, we have that
  \begin{align*}
w_h^{\pi\ind{1},\ldots,\pi\ind{t}}(x'\mid{}x,a)\ldef{}\frac{\Pmstar_{h-1}(x'\mid{}x,a)}{\sum_{i<t}d_h^{\sMstar,\pi\ind{i}}(x')+\Pmstar_{h-1}(x'\mid{}x,a)}
    \in \cW_h.
  \end{align*}
We assume without loss of generality that $\nrm*{w}_{\infty}\leq{}1$
for all $w\in\cW_h$.  
\end{assumption}
To compute a policy cover that approximately solves
$p_h=\argmin_{p\in\Delta(\PiRNS)}\pCovM[\Mstar](p_h)$ for parameter
$\veps>0$, we require that \cref{ass:weight_realizability_strong}
holds for $T=\frac{1}{\veps}$. Our guarantees can also be stated in
terms of the following weaker assumption, which is somewhat simpler to state.
\begin{assumption}[Weight function realizability---weak version]
  \label{ass:weight_realizability_weak}
  For all $h\geq{}2$ and all $\pi\in\PiNS$
  \begin{align*}
w_h^{\pi}(x'\mid{}x,a)\ldef{}\frac{\Pmstar_{h-1}(x'\mid{}x,a)}{d_h^{\sMstar,\pi}(x')}
    \in \cW_h.
  \end{align*}
\end{assumption}
The following result shows that \cref{ass:weight_realizability_weak}
implies \cref{ass:weight_realizability_strong}.
\begin{proposition}
  \label{prop:weight_realizability}
  For any $T\in\bbN$, given a weight function class $\cW$ satisfying
  \cref{ass:weight_realizability_weak}, the induced class $\cW'$ given by
  \begin{align*}
    \cW'_h\ldef
    \crl*{
    (x,a,x')\mapsto{}
    \frac{1}{1+\sum_{i<t}\frac{1}{w_h\ind{i}(x'\mid{}x,a)} 
    } \mid{} w_h\ind{1},\ldots,w_{h}\ind{t-1}\in\cW_h, t\in\brk{T}}
  \end{align*}
  satisfies \cref{ass:weight_realizability_strong}, and has $\log\abs*{\cW'_h}\leq\bigoh\prn*{T\cdot\log\abs*{\cW_h}}$.
\end{proposition}
For $T=\frac{1}{\veps}$ this
increases the weight function class size from $\log\abs*{\cW}$ to
$\bigoh\prn*{\frac{1}{\veps}\cdot\log\abs*{\cW}}$, leading to an extra
$\frac{1}{\veps}$ factor in the final sample complexity bound for our
main result. Consequently, we restrict our attention to
\cref{ass:weight_realizability_strong} going forward.

\cref{ass:weight_realizability_weak,ass:weight_realizability_strong}
are new to the best of our knowledge, and are naturally suited to the
pushforward coverability objective. While both assumption involve the
forward transition probability, they are significantly weaker than
model-based realizability because they only require modeling the
\emph{relative} transition probability, as the following example shows.
\begin{example}
  For a Block MDP  \citep{du2019latent,misra2019kinematic,zhang2022efficient,mhammedi2023representation}
  with latent state space $\cS$ and decoder class
  $\Phi\subseteq(\cX\to\cS)$, we can satisfy
  \cref{ass:weight_realizability_weak} with
  $\log\abs*{\cW}\leq\bigoht\prn{\abs*{\cS}^2\abs*{\cA}+\log\abs*{\Phi}}$,\footnote{Formally
    this requires a standard covering argument; we omit the details.}
  yet any realizable model class must have
  $\log\abs*{\cM}=\bigom(\abs*{\cX})\gg\abs*{\cS}$ in general.
\end{example}
See \citet{amortila2023harnessing} for further discussion around
weight function realizability in online reinforcement learning.



\paragraph{Weight function estimation subroutine}
\input{algorithm_weight_function}

Our weight function estimation subroutine, \estimateweight, is given
in \cref{alg:estimate_weight}. To motivate the algorithm, consider the
following abstract setting. Let $\cZ$ be a set. We receive samples
$\cD_1=\crl{z_\mu\ind{1},\ldots,z_\mu\ind{n}}\in\cZ$
and $\cD_2=\crl{z_\nu\ind{1},\ldots,z_\nu\ind{n}}\in\cZ$, where $z_\mu\ind{t}\sim\mu\ind{t}\in\Delta(\cZ)$ and
$z_\nu\ind{t}\sim\nu\ind{t}\in\Delta(\cZ)$. The distributions $\mu\ind{t}$ and $\nu\ind{t}$ can be chosen
in an adaptive fashion based on $z_\mu\ind{1},z_\nu\ind{1},\ldots,z_\mu\ind{t-1},z_\nu\ind{t-1}$. We define
$\mu=\frac{1}{n}\sum_{t=1}^{n}\mu\ind{t}$ and
$\nu=\frac{1}{n}\sum_{t=1}^{n}\nu\ind{t}$, and our goal is to estimate
the density ratio
\begin{align*}
  \wstar(z) \ldef \frac{\mu(z)}{\nu(z)}.
\end{align*}
Given \emph{realizable} weight function class $\cW$ with
$w^{\star}\in\cW$, \citet{nguyen2010estimating} (see also
\citet{katdare2023marginalized}) propose the estimator
\begin{align}
  \label{eq:weight_estimator_body}
\what \ldef \argmax_{w\in\cW} \Eh_{\cD_1}\brk*{\log(w)} - \Eh_{\cD_2}\brk*{w},
\end{align}
where $\Eh_\cD\brk{\cdot}$ denotes the empirical expectation with
respect to a dataset $\cD$. We show
(\cref{thm:weight_estimator_log} in \cref{app:model_free}) that this
estimator ensures that
\begin{align*}
  \En_{z\sim\nu}\brk[\big]{\prn[\big]{\sqrt{\what(z)}-\sqrt{w^{\star}(z)}}^2}
  \approxleq \bigoh(\nrm*{w^{\star}}_{\infty})\cdot\frac{\log(\abs{\cW}\delta^{-1})}{n}
\end{align*}
with high probability.

When invoked with layer $h\geq{}2$ and iteration $t\geq{}2$ within
\cref{alg:model_free}, \cref{alg:estimate_weight} simply sets $\cZ=\cX\times\cA\times\cX$ above and
collects datasets $\cD_1\sim\mu$ and $\cD_2\sim\nu$ such that
\begin{align*}
  \mu(x'\mid{}x,a)=\Pmstar_{h-1}(x'\mid{}x,a),\quad\nu(x'\mid{}x,a)=\frac{1}{t}\prn*{\sum_{i<t}d_h^{\sMstar,\pi\ind{h,i}}(x')
  + \Pmstar_{h-1}(x'\mid{}x,a)},
\end{align*}
and
\begin{align}
  \label{eq:roll_in_dist}
  \mu(x,a) = \nu(x,a) = \frac{1}{2}\prn*{d_{h-1}^{\sMstar,p_{h-1}}(x,a) + \frac{1}{t-1}\sum_{i<t}d_{h-1}^{\sMstar,\pi\ind{h,i}\circ_{h-1}\piunif}(x,a)}.
\end{align}
Then, in \cref{line:weight_alg}, the algorithm computes the estimator
\cref{eq:weight_estimator_body} with respect to the class
$t\cdot{}\cW$, which is guaranteed to have
\begin{align*}
  \frac{\mu(x,a,x')}{\nu(x,a,x')}
  = t\cdot{}w_h\ind{t}(x'\mid{}x,a) \in t\cdot{}\cW
\end{align*}
under \cref{ass:weight_realizability_strong}. The main guarantee for
this method is given in \cref{lem:weight_function_mf} in \cref{app:model_free}.

\paragraph{Policy optimization subroutine}
The policy optimization subroutine, \policyopt, is a hyperparameter to the algorithm,
and can be any subroutine that approximately solves the policy optimization problem
\begin{align*}
\pi\ind{h,t}\approx\argmax_{\pi\in\Pi}\En^{\sMstar,\pi}\brk*{
\what_h\ind{t}(x_h\mid{}x_{h-1},a_{h-1})},
\end{align*}
which treats the estimated weight function $\what_h\ind{t}$ as a
reward for layer $h-1$. \policyopt does not need to perform global
policy optimization---instead, we only require a certain form of
``local'' guarantee with respect to the approximate policy covers $p_{1},\ldots,p_{h-1}$.

To formalize the requirement of \policyopt, for each layer $h\geq{}2$ and iteration $t\in\brk{T}$, and each
$\ell\leq{}h-1$, we define
\begin{align*}
  Q_{\ell}^{\sMstar,\pi}(x,a;\what_h\ind{t})=\En^{\sMstar,\pi}\brk*{
  \what_h\ind{t}(x_h\mid{}x_{h-1},a_{h-1})\mid{}x_\ell=x,a_\ell=a
  }
\end{align*}
as the Q-function for a policy $\pi\in\PiNS$ under the (stochastic) reward
$r_{h-1}\ind{t}=\what_h\ind{t}(x_h\mid{}x_{h-1},a_{h-1})$ in
\cref{alg:model_free}. We assume that the policy
$\pi\ind{t,h}=\policyopt_{h-1}(r\ind{h,t}, p_{1:h-1},\eps,\delta)$
approximately maximizes this Q-function under $p_1,\ldots,p_{h-1}$.
\begin{assumption}
  \label{ass:policy_opt}
  For any fixed iteration $h\geq{}2$ and $t\in\brk{T}$, the subroutine
  $\policyopt_{h-1}(r\ind{h,t}, p_{1:h-1},\eps,\delta)$ produces a
  policy $\pi\ind{h,t}$ such that with probability at least $1-\delta$,
  \begin{align}
    \label{eq:policy_opt}
    \sum_{\ell=1}^{h-1}\En^{\sMstar,p_\ell}
  \brk*{\max_{a\in\cA}Q_{\ell}^{\sMstar,\pi\ind{h,t}}(x_\ell,a;\what_h\ind{t})
  -Q_{\ell}^{\sMstar,\pi\ind{h,t}}(x_\ell,\pi\ind{h,t}(x_\ell);\what_h\ind{t})}
    \leq \eps,
  \end{align}
  and does so using $\Nopt(\eps,\delta)$ episodes.
\end{assumption}
This assumption asserts that $\pi\ind{t,h}$ cannot be substantially
improved, but only with respect to the state distribution induced by
$p_1,\ldots,p_{h-1}$.\footnote{Note that if $p_1,\ldots,p_{h-1}$
  uniformly cover all policies, then \cref{ass:policy_opt} implies
  that $\pi\ind{h,t}$ is globally optimal by the performance
  difference lemma. However, \cref{eq:policy_opt} can still lead to
  useful guarantees in the presence of partial coverage, which our
  analysis critically exploits.}
This is a weak guarantee that can be achieved
using only data collected from $p_1,\ldots,p_{h-1}$ (e.g., via offline
RL methods or hybrid offline/online methods), and does not require
systematic exploration. 

\paragraph{\psdp as a policy optimization subroutine}
For concreteness, we make use of \psdp \citep{bagnell2003policy},
described in \cref{app:policy_opt} as the \policyopt subroutine. \psdp
optimizes a given reward function $r_{h-1}$ by collecting exploratory
data with $p_1,\ldots,p_{h-1}$ and applying approximate dynamic
programming with a user-specified value function class $\cQ$. We make the following
value-based realizability assumption, which asserts that $\cQ$ is
expressive enough to allow \psdp to optimize any weight function in
the class $\cW$.
\begin{assumption}
  \label{ass:qpi_weight}
  We have access to a value function class $\cQ=\cQ_{1:H}$ with
  $\cQ_h\subseteq(\cX\times\cA\to\brk{0,1})$ such that for all
  $h\in\brk{H}$, $w\in\cW_h$, and $\pi\in\PiNS$, we have
  $Q_\ell^{\sMstar,\pi}(\cdot,\cdot;w)\in\cQ_\ell$ for all $\ell\leq{}h-1$, where 
  \begin{align*}
  Q_{\ell}^{\sMstar,\pi}(x,a;w)=\En^{\sMstar,\pi}\brk*{
  w_h(x_h\mid{}x_{h-1},a_{h-1})\mid{}x_\ell=x,a_\ell=a
  }
  \end{align*}
  is the Q-function for $\pi$ under the (stochastic) reward
$r_{h-1}=w(x_h\mid{}x_{h-1},a_{h-1})$.
\end{assumption}

      \begin{lemma}[Local optimality for \psdp]
        \label{lem:psdp_simple}
        Suppose \cref{ass:qpi_weight} holds. Then for any $\eps,\delta\in(0,1)$, the subroutine
        $\pi\ind{h,t}=\psdp_{h-1}(r\ind{h,t}, p_{1:h-1},\eps,\delta)$
        satisfies \cref{ass:policy_opt}, and does so using at most
        $\Npsdp(\eps,\delta)=\bigoh\prn*{\frac{H^3\abs*{\cA}\log(\abs{\cQ}H\delta^{-1})}{\eps^2}}$ episodes.
      \end{lemma}
      See \cref{app:policy_opt} for details.
We expect that similar guarantees can be proven for Natural Policy
Gradient, Conservative Policy Iteration, and other standard local
search methods. Different subroutines may allow one to make use of
weaker function approximation requirements.

\subsection{Main Result}

The main guarantee for \cref{alg:model_free} is as follows.

\begin{restatable}[Main result for \cref{alg:model_free}]{theorem}{modelfree}
  \label{thm:model_free}
  Let $\veps\in(0,1/2)$ and $\delta\in(0,e^{-1})$ be given, and suppose that \cref{ass:weight_realizability_strong} and
  \cref{ass:policy_opt} are satisfied. Then \cref{alg:model_free}
  produces policy covers $p_1,\ldots,p_H\in\Delta(\PiRNS)$ such that with probability at least $1-\delta$, for all $h\in\brk{H}$,
\[
  \pCovM[\Mstar](p_h)   \leq{} 170H\log(\veps^{-1})\cdot{}\CpushM[\Mstar],
\]
and does so using at most 
\begin{align*}
  N \leq \bigoht\prn*{\frac{H\abs*{\cA}\log(\abs{\cW}\delta^{-1})}{\veps^3}
  +\frac{H}{\veps}\Nopt(c\veps^2,\delta/2HT)}
\end{align*}
episodes, where $c>0$ is a sufficiently small absolute constant.
\end{restatable}
In particular, this result shows that we can optimize the pushforward
coverability objective (and consequently the \mainobj objective, via
\cref{prop:pushforward_relaxation}), up to small
$\bigoh(H\log(\veps^{-1}))$ approximation factor. The sample
complexity is polynomial in all relevant problem parameters whenever
the subroutine \policyopt has polynomial sample complexity.


\paragraph{Guarantee for \mfalg with \psdp}
Combining \cref{thm:model_free} with the guarantee for \psdp (\cref{lem:psdp_simple}), we obtain the
following corollary.
\begin{corollary}[Main result for \cref{alg:model_free} with \psdp]
  \label{cor:model_free_psdp}
    Let $\veps\in(0,1/2)$ and $\delta\in(0,e^{-1})$ be given, and
    suppose that we have a weight function class $\cW$ and value
    function class $\cQ$ such that \cref{ass:weight_realizability_strong,ass:qpi_weight} are satisfied. Then with
  \psdp (\cref{alg:psdp}) as a policy optimization subroutine, \cref{alg:model_free}
  produces policy covers $p_1,\ldots,p_H\in\Delta(\PiRNS)$ such that with probability at least $1-\delta$, for all $h\in\brk{H}$,
\[
  \pCovM[\Mstar](p_h)   \leq{} 170H\log(\veps^{-1})\cdot{}\CpushM[\Mstar],
\]
and does so using at most 
\begin{align*}
  N \leq \bigoht\prn*{\frac{H\abs*{\cA}\log(\abs{\cW}\delta^{-1})}{\veps^3}
        +\frac{H^4\abs*{\cA}\log(\abs{\cQ}\delta^{-1})}{\veps^5}}
\end{align*}
episodes.
\end{corollary}

Let us discuss some key features of this result.
\begin{itemize}
\item \emph{Sample efficiency.} The sample complexity in \cref{cor:model_free_psdp} scales as
  $\poly(H,\abs*{\cA},\log\abs{\cW},\log\abs*{\cQ},\veps^{-1})$, and
  hence is efficient for large state spaces; we
  expect that the precise polynomial factors can be tightened, as can
  the approximation ratio in the objective value, though we leave this
  for future work. As with our results in preceding sections, the
  resulting policy covers $p_1,\ldots,p_H$ can be directly used for
  downstream policy optimization.
\item \emph{Computational efficiency.} With \psdp as the \policyopt subroutine, \cref{alg:model_free}
  is computationally efficient whenever i) the weight function
  estimation objective in \cref{line:weight_alg} of
  \cref{alg:estimate_weight} can be solved efficiently over $\cW$, and
  ii) square loss regression over the class $\cQ$ can be solved
  efficiently. We consider these to be fairly mild assumptions.
\item \emph{Practicality.} In practice, we expect that the subroutine
  \policyopt can be implemented using off-the-shelf deep RL methods
  (e.g., PPO or SAC), which are known to perform well given access to
  exploratory data. In this sense, \cref{alg:model_free} can be viewed
  as a new approach to equipping existing deep RL methods with
  exploration, with the weight function-based rewards in
  \cref{line:mf_reward} acting as exploration bonuses.
\end{itemize}

As a concrete example, we can instantiate \cref{cor:model_free_psdp}
for Block MDPs to derive end-to-end guarantees under standard assumptions.
\begin{example}[Sample complexity for Block MDP]
    For a Block MDP  \citep{du2019latent,misra2019kinematic,zhang2022efficient,mhammedi2023representation}
  with latent state space $\cS$ and decoder class
  $\Phi\subseteq(\cX\to\cS)$, we can satisfy
  \cref{ass:weight_realizability_weak} with
  $\log\abs*{\cW}\leq\bigoht\prn{\abs*{\cS}^2\abs*{\cA}+\log\abs*{\Phi}}$
  and $\log\abs*{\cQ}\leq\bigoht\prn{\abs*{\cS}\abs*{\cA}+\log\abs*{\Phi}}$,
  so \cref{cor:model_free_psdp} gives sample complexity
  $N \leq \bigoht\prn*{\frac{H^4\abs*{\cS}^2\abs*{\cA}^2\log(\abs{\Phi}\delta^{-1})}{\veps^5}}$.
\end{example}

We view the results in this section as a proof-of-concept, showing
that the iterative \mainobj optimization methods in
\cref{sec:planning} can be implemented in a sample-efficient
fashion. We leave sample-efficient counterparts to other relaxations
for future work.

\subsection{Additional details on subroutines}









==> widebar.tex <==

\makeatletter
\let\save@mathaccent\mathaccent
\newcommand*\if@single[3]{%
  \setbox0\hbox{${\mathaccent"0362{#1}}^H$}%
  \setbox2\hbox{${\mathaccent"0362{\kern0pt#1}}^H$}%
  \ifdim\ht0=\ht2 #3\else #2\fi
  }
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
\newcommand*\widebar[1]{\@ifnextchar^{{\wide@bar{#1}{0}}}{\wide@bar{#1}{1}}}
\newcommand*\underbar[1]{\@ifnextchar_{{\under@bar{#1}{0}}}{\under@bar{#1}{1}}}
\newcommand*\wide@bar[2]{\if@single{#1}{\wide@bar@{#1}{#2}{1}}{\wide@bar@{#1}{#2}{2}}}
\newcommand*\under@bar[2]{\if@single{#1}{\under@bar@{#1}{#2}{1}}{\under@bar@{#1}{#2}{2}}}
\newcommand*\wide@bar@[3]{%
  \begingroup
  \def\mathaccent##1##2{%
    \let\mathaccent\save@mathaccent
    \if#32 \let\macc@nucleus\first@char \fi
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
    \ifdim\dimen@>\z@ \dimen@0pt\fi
    \rel@kern{0.6}\kern-\dimen@
    \if#31
      \overline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
      \advance\dimen@0.4\dimexpr\macc@kerna
      \let\final@kern#2%
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      \overline{\rel@kern{-0.6}\kern\dimen@#1}%
    \fi
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
  \if#31
    \macc@nested@a\relax111{#1}%
  \else
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
  \fi
  \endgroup
}
\newcommand*\under@bar@[3]{%
  \begingroup
  \def\mathaccent##1##2{%
    \let\mathaccent\save@mathaccent
    \if#32 \let\macc@nucleus\first@char \fi
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
    \ifdim\dimen@>\z@ \dimen@0pt\fi
    \rel@kern{0.6}\kern-\dimen@
    \if#31
      \underline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
      \advance\dimen@0.4\dimexpr\macc@kerna
      \let\final@kern#2%
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      \underline{\rel@kern{-0.6}\kern\dimen@#1}%
    \fi
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
  \if#31
    \macc@nested@a\relax111{#1}%
  \else
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
  \fi
  \endgroup
}
\makeatother


